A novel analysis of utility in privacy pipelines, using Kronecker products and quantitative information flow

We combine Kronecker products, and quantitative information flow, to give a novel formal analysis for the fine-grained verification of utility in complex privacy pipelines. The combination explains a surprising anomaly in the behaviour of utility of privacy-preserving pipelines -- that sometimes a reduction in privacy results also in a decrease in utility. We use the standard measure of utility for Bayesian analysis, introduced by Ghosh at al., to produce tractable and rigorous proofs of the fine-grained statistical behaviour leading to the anomaly. More generally, we offer the prospect of formal-analysis tools for utility that complement extant formal analyses of privacy. We demonstrate our results on a number of common privacy-preserving designs.

==> macrosForCCM.tex <==
% !TEX root = CCMonDP.tex

\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

\newcommand\In {:}
\newcommand\Wide[1] {\quad#1\quad}
\newcommand\Defs {:=}
\newcommand\Eqs {~~=~~}

\newcommand\Apply {\triangleright}
\newcommand\Dist {\mathbb{D}}
\newcommand{\DDist} {\Dist^2}
\newcommand\Hyper[2]  {[#1{\Apply}#2]}
\newcommand\Leak {\mathcal{L}}
\newcommand\mult    {\times}
\newcommand\RealNN {\mathbb{R}_{\geq 0}}

\newcommand\uniform {\upsilon}
\newcommand\ChanRef {\sqsubseteq}

\newcommand\Eqn[1] {Eqn~(\ref{#1})}
\newcommand\Thm[1] {Thm~\ref{#1}}
\newcommand\Lem[1] {Lem~\ref{#1}}
\newcommand\Def[1] {Defn~\ref{#1}}
\newcommand\Alg[1] {Alg.~\ref{#1}}

\newcommand\calx {\mathcal{X}}
\newcommand\caly {\mathcal{Y}}
\newcommand\calz {\mathcal{Z}}
\newcommand\calu {\mathcal{U}}
\newcommand\calw {\mathcal{W}}

% Kronecker
\newcommand\kron   {\otimes}
\newcommand\nfold[2] { #2^{\kron #1}}


%%
%% end of the preamble, start of the body of the document source.
\newenvironment{Reason}{\vspace{-.0em}\begin{tabbing}\hspace{2em}\= \hspace{1cm} \= \kill}
    {\end{tabbing}\vspace{-1em}}
\newcommand\Step[2] {#1 \> $\begin{array}[t]{@{}llll}#2\end{array}$ \\}
\newcommand\StepR[3] {#1 \> $\begin{array}[t]{@{}llll}#3\end{array}$
    \` {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\WideStepR[3] {#1 \>
    $\begin{array}[t]{@{}ll}~\\#3\end{array}$ \`
    {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\RF {\small}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% General macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\qm}[1]{``#1''}

%%% 0835: Carroll's macros.
\newcommand\Cite[1] {{\textcolor{red}{[#1]}}}
\newcommand\XX {\ensuremath{\mathcal X}}
\newcommand\YY {\ensuremath{\mathcal Y}}
\newcommand\DP {\textit{DP}}
\newcommand\EDP {\VE-\textit{DP}}
\newcommand\VEC {\VE-close}
\newcommand\VE {\ensuremath{\varepsilon}}
%\newcommand\GM {\ensuremath{\mathit{GM}}}
%\newcommand\RR {\ensuremath{\mathit{RR}}}
\newcommand\RR[1][] {\ensuremath{\ifx\empty#1\empty{\mathit RR}_p     \else {\mathit RR}_{#1}\fi}} %%%
\newcommand\GD[1][]   {\ensuremath{\ifx\empty#1\empty{\mathit GD}_\alpha\else {\mathit GD}_{#1}\fi}} %
\newcommand\Forr {{\sf pro}}
\newcommand\Against {{\sf anti}}
\newcommand\MM {\ensuremath{\,{\cdot}\,}} % Martrix multiplication.
\newcommand\Fun {{\rightarrow}\;}
\newcommand\Nat {\ensuremath{\naturals}}
\newcommand\Real {\ensuremath{\reals}}
\newcommand\NF[2] {\ensuremath{\nicefrac{#1}{#2}}}
\newcommand\WIDE[1] {\quad\quad#1\quad\quad}
% 0835


\newcommand{\domainofdatasets}{\cald}

\newcommand{\attrset}{\cala}

\newcommand{\domainofrows}[1]{\textit{rows}(#1)}
\newcommand{\rowprior}{\pi^{\star}}
\newcommand{\rowpriorgivend}{\pi^{\domainofrows{\attrset}^{\star}{\mid}D}}

\newcommand{\attrprior}[1]{\pi^{\star#1}}
\newcommand{\attrpriorgivend}[1]{\pi^{\star#1^{\mid}D}}

\newcommand{\senscol}{a_{s}}
\newcommand{\sensset}{\domain{\senscol}}
\newcommand{\sensprior}{\attrprior{\senscol^{\star}}}
\newcommand{\senspriorgivend}{\attrpriorgivend{\senscol}}

\newcommand{\usefulcol}{a_{u}}
\newcommand{\usefulset}{\domain{\usefulcol}}
\newcommand{\usefulprior}{\attrprior{\usefulcol}}
\newcommand{\usefulpriorgivend}{\attrpriorgivend{\usefulcol}}

\newcommand{\countpropprior}[1]{\pi^{\countprop(#1)}}
\newcommand{\countproppriorgivend}[1]{\pi^{\countprop(#1){\mid}D}}

\newcommand{\countquery}[1]{\texttt{count}_{q}}
\newcommand{\countprop}{\countquery{\prop}}

\newcommand{\privloss}{\textit{privacy{-}loss}}
\newcommand{\priorvul}{\textit{prior{-}vul}}
\newcommand{\postvul}{\textit{post{-}vul}}
\newcommand{\utility}{\textit{utility}}
\newcommand{\utilityloss}{\textit{utility{-}loss}}

\newcommand{\range}[1]{\textit{range}(#1)}

\newcommand{\context}{\Gamma}
\newcommand{\contextobv}{\Gamma^{\textit{obv}}}
\newcommand{\contextloc}{\Gamma^{\textit{loc}}}

\newcommand{\lossfunc}{\ell}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Math macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cala}{\mathcal{A}}
\newcommand{\calc}{\mathcal{C}}
\newcommand{\cald}{\mathcal{D}}
\newcommand{\calr}{\mathcal{R}}
\newcommand{\cals}{\mathcal{S}}

\newcommand{\dist}{\mathbb{D}}

\newcommand*{\ldblbrace}{\{\mskip-5mu\{}
\newcommand*{\rdblbrace}{\}\mskip-5mu\}}
\newcommand{\multiset}[1]{\ldblbrace#1\rdblbrace}
\newcommand{\multiplicity}[2]{m_{#1}(#2)}

\newcommand{\domain}[1]{\mathit{domain}(#1)}
\newcommand{\equivrel}[1]{\sim_{#1}}
\newcommand{\equivclass}[1]{\textit{equiv{-}class}({#1})}
\newcommand{\equivclasslong}[2]{\textit{equiv{-}class}^{#1}({#2})}
\newcommand{\partition}[2]{{#1}{/}_{#2}}

\newcommand{\bool}{\texttt{Bool}}
\newcommand{\true}{\texttt{true}}
\newcommand{\false}{\texttt{false}}

\newcommand{\naturals}{\mathbb{N}}
\newcommand{\reals}{\mathbb{R}}

\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Model macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\query}{f}
\newcommand{\mech}{M_{\countprop}}
\newcommand{\mechobv}{\mech^{\textit{obv}}}
\newcommand{\mechloc}{\mech^{\textit{loc}}}
\newcommand{\rand}{R}
% \newcommand{\rands}{\rand^{\cals}}
% \newcommand{\randu}{\rand^{\calu}}
\newcommand{\randobv}{\rand^{\textit{obv}}}
\newcommand{\randloc}{\rand^{\textit{loc}}}
\newcommand{\prop}{q}

\newcommand{\distcontext}{p^{\context}}
\newcommand{\distobv}{p^{\contextobv}}
\newcommand{\distloc}{p^{\contextloc}}

\newcommand{\dirac}[2]{\delta_{#1}(#2)}

\newcommand{\priv}[2]{\textit{privacy}(#1,#2)}
\newcommand{\util}[2]{\textit{utility}(#1,#2)}

\newcommand{\randomize}[1]{\textit{rand}(#1)}

\newcommand{\xstar}{x^{\star}}
\newcommand{\extgen}[2]{#1{\cup}#2}
\newcommand{\extd}[1]{\extgen{D}{#1}}
\newcommand{\dstar}{\extd{\xstar}}
\newcommand{\dx}{\extd{x}}
\newcommand{\dy}{\extgen{d}{y}}

\newcommand{\indu}{w}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Macros for weird behavior on utility example
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\custody}{\textit{custody}}

\newcommand{\gainfunc}{g}
\newcommand{\gid}{g_{\textit{id}}}
\newcommand{\utilitygain}{\textit{utility{-}gain}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
